Piccolo: Large-Scale Graph Processing with Fine-Grained In-Memory Scatter-Gather

Graph processing requires irregular, fine-grained random access patterns incompatible with contemporary off-chip memory architecture, leading to inefficient data access. This inefficiency makes graph processing an extremely memory-bound application. Because of this, existing graph processing accelerators typically employ a graph tiling-based or processing-in-memory (PIM) approach to relieve the memory bottleneck. In the tiling-based approach, a graph is split into chunks that fit within the on-chip cache to maximize data reuse. In the PIM approach, arithmetic units are placed within memory to perform operations such as reduction or atomic addition. However, both approaches have several limitations, especially when implemented on current memory standards (i.e., DDR). Because the access granularity provided by DDR is much larger than that of the graph vertex property data, much of the bandwidth and cache capacity are wasted. PIM is meant to alleviate such issues, but it is difficult to use in conjunction with the tiling-based approach, resulting in a significant disadvantage. Furthermore, placing arithmetic units inside a memory chip is expensive, thereby supporting multiple types of operation is thought to be impractical. To address the above limitations, we present Piccolo, an end-to-end efficient graph processing accelerator with fine-grained in-memory random scatter-gather. Instead of placing expensive arithmetic units in off-chip memory, Piccolo focuses on reducing the off-chip traffic with non-arithmetic function-in-memory of random scatter-gather. To fully benefit from in-memory scatter-gather, Piccolo redesigns the cache and MHA of the accelerator such that it can enjoy both the advantage of tiling and in-memory operations. Piccolo achieves a maximum speedup of 3.28$\times$ and a geometric mean speedup of 1.62$\times$ across various and extensive benchmarks.

==> algo/vcm.tex <==
\SetInd{0.6em}{0.7em}
\setlength{\algomargin}{8pt}
\begin{algorithm}[t]
%\footnotesize
%\scriptsize
    \caption{Vertex-Centric Model (VCM)}
    \label{algo:vcm}
    \DontPrintSemicolon
    \SetNoFillComment
    \SetKwBlock{DoParallel}{do in parallel}{end}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwProg{Fn}{Function}{}{end}
    \Input{$G=(V,E)$}
    \For{\textbf{\upshape $v$} $\in$ \textbf{\upshape $G.V$}}
    {
        \For{$e$ $\in$ \upshape $v$.outEdges}
        {
            $res$ = \textbf{process}($e$.weight, $v$.value)
            \textit{\textcolor{gray}{\ \ \  //\ \circled{1} process}}\; 
            u.temp = \textbf{reduce}(u.temp, res)
            \textit{\textcolor{gray}{\ \ \ \ \ \ \ //\ \circled{2} reduce}}\;  
        }
    }
    \For{\textbf{\upshape $v$} $\in$ \textbf{\upshape $G.V$}}
    {
        v.value = \textbf{apply}(v.temp, v.value)
        \textit{\textcolor{gray}{\ \ \ \ \ \ \ //\ \circled{3} apply}}\; 
    }
\end{algorithm}

==> bak_cost.tex <==



bandwidth utilization but not the locality.
In line 5, reading $V_{temp}$ randomly spans across the entire array.
If all vertices are active and $V_{temp}$ is sufficiently larger than the cache, the total number of accesses $M_{base}$ becomes
\begin{equation}
%\begin{medsize}
\begin{aligned}
    M_{base} &= (|V| + |E|) + c\cdot|E| + |V|.
\end{aligned}
\label{eq:base}
%\end{medsize}
\end{equation}
The first term is for accessing topology in CSR format, the second term is for randomly reading $V_{temp}$ where $c$ is the burst size, and the third term is for updating the vertices. 

A popular technique is graph tiling~\cite{mosaic,flashgraph,gridgraph}, which involves limiting the range of outgoing neighbors and thus splitting the $V_{prop}$ array into tiles. The memory cost $M_{tile}$ is
\begin{equation}
%\begin{medsize}
\begin{aligned}
    M_{tile} &= (t\cdot|V| + |E|) + t\cdot c\cdot |E|\cdot r(|V|/t) + |V|,
\end{aligned}
\label{eq:tile}
%\end{medsize}
\end{equation}
where $t$ is the number of tiles, which accounts for the vertex indices per tile, and repeated loading of $V_{prop}$ tiles into the cache.
We assume that the miss rate $r()$ is a function of the tile size.
Specifically, when the tile is small enough to fit the cache, it is called \emph{perfect tiling} that only involves cold misses (i.e., $r=|V|/c|E|$):
\begin{equation}
%\begin{medsize}
\begin{aligned}
    M_{perfect} &= (t\cdot|V| + |E|) + t\cdot|V| + |V|.
\end{aligned}
\label{eq:perfect}
%\end{medsize}
\end{equation}

Because $r()$ quickly decreases with larger $t$, tiling is an effective approach, where the perfect tiling is preferred in many cases.
However, there are several cases where slightly larger tiles are beneficial. 
This happens when only a subset of vertices are active, $t$ is too large due to the graph size, or $c$ is small due to small burst size of the memory.
